Cost Design in Atomic Routing Games

An atomic routing game is a multiplayer game on a directed graph. Each player in the game chooses a path -- a sequence of links that connect its origin node to its destination node -- with the lowest cost, where the cost of each link is a function of all players' choices. We develop a novel numerical method to design the link cost function in atomic routing games such that the players' choices at the Nash equilibrium minimize a given smooth performance function. This method first approximates the nonsmooth Nash equilibrium conditions with smooth ones, then iteratively improves the link cost function via implicit differentiation. We demonstrate the application of this method to atomic routing games that model noncooperative agents navigating in grid worlds.

==> routing/graph.tex <==
\begin{figure}[!ht]
    \centering
    \tikzset{
    node/.style={circle,draw,minimum size=0.5em},
    link/.style={->,> = latex'}
}
    \begin{tikzpicture}[scale=0.4]
    
   \node[node] at (0, 0) (1) {\scriptsize \color{red}1}; 
   \node[node] at (4, -1.73) (2) {\scriptsize \color{red}2}; 
   \node[node] at (4, 1.73) (3) {\scriptsize \color{red}3}; 
   \node[node] at (8, 0) (4) {\scriptsize \color{red}4}; 
   
   \draw[link] (1) -- node[midway, label={[label distance=-0.5cm,text depth=2ex, rotate=-30]above: {\scriptsize \color{blue} 1}}] {} (2);
   \draw[link] (1) -- node[midway, label={[label distance=-0.5cm,text depth=2ex, rotate=30]above: {\scriptsize \color{blue} 2}}] {} (3);
   \draw[link] (2) -- node[midway, label={[label distance=-0.5cm,text depth=2ex, rotate=30]above: {\scriptsize \color{blue} 3}}] {} (4);
   \draw[link] (3) -- node[midway, label={[label distance=-0.5cm,text depth=2ex, rotate=-30]above: {\scriptsize \color{blue} 4}}] {} (4);
   \draw[link] (2) to[bend left=15]node[midway, label={[label distance=0,text depth=1ex]left: {\scriptsize \color{blue} 5}}] {} (3);
   \draw[link] (3) to[bend left=15]node[midway, label={[label distance=0,text depth=1ex]right: {\scriptsize \color{blue} 6}}] {} (2);

    \end{tikzpicture} 
    \caption{A directed graph with node and link labels.}
    \label{fig: graph}
\end{figure}
